PsyEval: A Suite of Mental Health Related Tasks for Evaluating Large Language Models

Evaluating Large Language Models (LLMs) in the mental health domain poses distinct challenged from other domains, given the subtle and highly subjective nature of symptoms that exhibit significant variability among individuals. This paper presents PsyEval, the first comprehensive suite of mental health-related tasks for evaluating LLMs. PsyEval encompasses five sub-tasks that evaluate three critical dimensions of mental health. This comprehensive framework is designed to thoroughly assess the unique challenges and intricacies of mental health-related tasks, making PsyEval a highly specialized and valuable tool for evaluating LLM performance in this domain. We evaluate twelve advanced LLMs using PsyEval. Experiment results not only demonstrate significant room for improvement in current LLMs concerning mental health but also unveil potential directions for future model optimization.

==> contents/limitations.tex <==
% !TEX root = ../main.tex

\section{Limitations}

While our study contributes valuable insights to the evaluation and understanding of LLMs in the context of mental health, it is essential to acknowledge certain limitations that affect the scope and generalizability of our findings.

The benchmark tasks were designed based on existing datasets, and thus, the performance of LLMs is contingent on the characteristics and biases present in those datasets. Addressing the broader diversity of mental health scenarios and cultural contexts might require more comprehensive and diverse datasets.

Our benchmark primarily focuses on specific tasks related to mental health, and the performance may not fully capture the complexities of real-world clinical scenarios. The translation from benchmark tasks to actual clinical applications might require additional considerations.

While our study touches upon the models' limited understanding of empathy and dialogue safety, a more in-depth analysis of these aspects is needed. Understanding the ethical implications and potential risks associated with LLMs in mental health applications requires dedicated research.
